Tensor Methods for Additive Index Models under Discordance and Heterogeneity

Motivated by the sampling problems and heterogeneity issues common in high- dimensional big datasets, we consider a class of discordant additive index models. We propose method of moments based procedures for estimating the indices of such discordant additive index models in both low and high-dimensional settings. Our estimators are based on factorizing certain moment tensors and are also applicable in the overcomplete setting, where the number of indices is more than the dimensionality of the datasets. Furthermore, we provide rates of convergence of our estimator in both high and low-dimensional setting. Establishing such results requires deriving tensor operator norm concentration inequalities that might be of independent interest. Finally, we provide simulation results supporting our theory. Our contributions extend the applicability of tensor methods for novel models in addition to making progress on understanding theoretical properties of such tensor methods.

==> background.tex <==
%!TEX root =main.tex


\section{Background and Model Definition}\label{sec:models}

\begin{definition}[Mixture of SIMs] \label{def:sim}
  Let $Z \in \{ 1, \ldots, k \}$ be a discrete random variable  such that $\PP(Z = j) = \pi_j $ for each $j \in [k]$.
  Let $X\sim N( 0 , I_d) $ be the covariate. Given $Z = j$, the reponse variable is given by 
  $Y = f_j( \la X , \beta^{*}_j\ra,  \epsilon)$,
  where $\epsilon \in \RR$ is the random noise which is indepedent of both $Z$ and $X$, and $f_j \colon\RR^2 \rightarrow \RR $ is a bivariate link function which is unknown.
\end{definition}
Note that the norm of $\beta^{*}_j$ can be absorbed in the unknown function $f_j$, thus not identifiable. We assume that $\beta^{*}_j$ have norm one for all $j \in [k]$ to make the model partially identifiable. Furthermore, we assume that the number of mixture components $k$ can be larger than the dimensionality $d$, which is means that the model in \eqref{def:sim} is overpametrized. 

\begin{definition} [A more general version]
  Let $X \in \RR^d$ be the covariate which has standard Gaussian distribution. Given $X =x$, we assume that a discrete random variable $Z \in \{ 1, \ldots, k \}$ is distributed according to $\PP( Z = j | X = x) = \pi_j (\la \beta_j^*,  x \ra )$ for any $j \in [k]$. Here we assume that $\sum_{j\in[k]} \pi_j(u) = 1$ for any $u \in \RR$. Moreover, given $Z=j$ and $X = x$, the response variable is given by 
  $Y = f_j (\la \beta_j^*, x \ra, \epsilon )$, where $\epsilon \in \RR$ is the random noise which is indepedent of both $Z$ and $X$, and $f_j \colon\RR^2 \rightarrow \RR $ is a bivariate link function which is unknown. 
\end{definition}


{\color{red} Introduce the overparametrized problem, which needs parameter identification.}














==> tensorconc.tex <==
%!TEX root =main.tex

\section{Tensor Concentration Results} \label{sec:tenconc}
As mentioned in \S\ref{sec:theory}, in order to obtain our main results in Theorem~\ref{thm:ldrates}, we require concentration bounds on $\| \hat M_1 - \EE [ h_1(\mathcal{Z}) \cdot S_3(X)] \|_{\oper}$ and $\| \hat M_2 - \EE [ h_2(\mathcal{Z}) \cdot S_3(X)] \|_{\oper}$. Similarly, to prove Theorem~\ref{thm:hdrates} we require concentration bounds for $\| \hat M_1 - \EE [ h_1(\mathcal{Z}) \cdot S_3(X)] \|_{\oper,r}$ and $\| \hat M_2 - \EE [ h_2(\mathcal{Z}) \cdot S_3(X)] \|_{\oper,r}$. Our main contribution in this paper is obtaining such bounds for the case of the model consider in Definitions~\ref{def:sim0} and~\ref{def:sim} . Compared to the matrix concentration results, obtaining concentration results for higher-order tensors are significantly challenging. The main difficulty is obtaining sharp concentration bounds for certain polynomial functions of random variables, that enables one to leverage the $\epsilon$-netting combined with union bound argument. %We refer the reader to~\cite{vershynin2010introduction} for a discussion on the definition of sub-Gaussian or sub-exponential random variables and the associated %In what follows, characterize the concentration of $\hat T$ to $\EE [ Y \cdot S_3(X)]$ in the both the tensor operator norm and the sparse tensor operator norm.

{\bf Q: Should move to previous section}


\begin{theorem} \label{thm:tensor_concentration}
Note that we define tensors   $\hat M_1$ and $\hat M_2$   in \eqref{eq:moment_tensor1} and \eqref{eq:moment_tensor2}, respectively.   Under Assumption \ref{assume:moments}, with probability at least $1 -\exp(-2d)$,  we have
 \#\label{eq:tensor_concentration}
&  \max \Bigl \{  \bigl \| \hat M_1 - \EE [ h_1(\mathcal{Z}) \cdot S_3(X)]  \bigr \|_{\oper} , \bigl \| \hat M_2 - \EE [ h_2(\mathcal{Z}) \cdot S_3(X)] \bigr \|_{\oper} \Bigr \} \notag \\
  &\qquad \leq  K_{  1} \max  \bigl ( \sqrt{d/ n},  d^{5/2}/ n  \bigr)
 + K_{2}  \max \bigl( \sqrt{ d/n },  d^{3/2}/n  \bigr ) ,
 \#
 where $K_{1}$ and $K_2$ are absolute constants.  {\bf Q: one model or two?}
\end{theorem}
\noindent The above theorem, establishes concentration of  $\hat M_1 - \EE [ h_1(\mathcal{Z}) \cdot S_3(X)]$ and $\hat M_2 - \EE [ h_2(\mathcal{Z}) \cdot S_3(X)]$ in tensor operator norm.  We now establish  the sparse tensor operator norm bounds.

%\textcolor{red}{todo}%\subsection{Sparse Tensor Operator Norm Bounds}

\begin{theorem} \label{thm:tensor_concentration1}
Under  Assumption~\ref{assume:moments}, with probability at least $1 - 8 \exp[ - 3r \log (d/r) ] $, we have
 \#%\label{eq:tensor_concentration}
 &  \max \Bigl \{  \bigl \| \hat M_1 - \EE [ h_1(\mathcal{Z}) \cdot S_3(X)]  \bigr \|_{\oper} , \bigl \| \hat M_2 - \EE [ h_2(\mathcal{Z}) \cdot S_3(X)] \bigr \|_{\oper} \Bigr \} \notag \\
& \qquad\leq K_{3} \cdot \max \bigl \{     [  r \log (d/r )/ n    ]^{1/2},   [  r \log (d/r) ]^{5/2}/ n  \bigr \}  \notag \\
&\qquad \qquad+  K_{4} \cdot  \max \bigl\{  [  r \log (d/r )/n    ]^{1/2},   [  r \log (d/r) ]^{3/2}/ n  \bigr \} , \label{eq:stopt2}
 \#
 where $r$ is a positive integer (typically much less than $d$) and $K_{3}$ and $K_{4}$ are absolute constants.
 {\bf Q: what makes the difference? Isn't $\log(d/r) = \log d$?}
\end{theorem}

We now prove the above two theorems. Auxiliary results required in the proof are provided in Appendix~\ref{sec:aux}.%

%\begin{theorem} \label{thm:tensor_concentration2}
%Let $r$ be an integer. With probability at least $1 - 8 \exp[ - 3r \log (d/r) ] $, we have
% \#\label{eq:tensor_concentration}
% \bigl \| \hat T - \EE ( \hat T) \bigr \|_{\oper, r}  &\leq K_{T_1} \cdot \max \biggl \{ \biggl [ \frac{r \log (d/r )}{n} \biggr ]^{1/2}, \frac{ [  r \log (d/r) ]^{5/2}} {n} \biggr \} \notag \\
 %&\quad +  K_{T_2} \cdot  \max \biggl \{ \biggl [ \frac{r \log (d/r )}{n} \biggr ]^{1/2}, \frac{ [  r \log (d/r) ]^{3/2}} {n} \biggr \} ,
% \#
% where $K_{T_1}$ and $K_{T_2}$ are absolute constants.

%\end{theorem}


\subsection{Proof of Theorem \ref{thm:tensor_concentration}}\label{sec:proof_thm1}

In this section, we present the   proof of Theorem \ref{thm:tensor_concentration}.
  Since the results for $\hat M_1$ and $\hat M_2$    are established using similar techniques, in the following, we first present a detailed proof of the bound on     $\| \hat M_2 - \EE [ h_2(\mathcal{Z}) \cdot S_3(X)]\|_{\oper}$, then prove the other part by showing the differences.

\vspace{10pt}
{\noindent \bf Upper bound for  $\| \hat M_2 - \EE [ h_2(\mathcal{Z}) \cdot S_3(X)]\|_{\oper}$.}
First note that by the definition of third order score function $S_3$ in \eqref{eq:3rd_score},   we have
$
\hat M_2 = \hat T_1+ \hat T_2 ,
$
where $\hat M_2$ is given in \eqref{eq:moment_tensor2}, and we define $\hat T_1$ and $\hat T_2$ respectively  by
\#
& \hat T_1 = \frac{1}{n} \sum_{i=1}^n Y^{(i)}  \cdot X^{(i)} \otimes X^{(i)} \otimes X^{(i)}, \label{eq:def_T1} \\
& \hat T_2 = \frac{1}{n} \sum_{i=1}^n \sum_{j=1}^d Y^{(i)}  \cdot \bigl  ( X^{(i)} \otimes e_j \otimes e_j +e_j \otimes X^{(i)}\otimes e_j + e_j \otimes e_j \otimes X^{(i)} \bigr ) \label{eq:def_T2},
\#
where    $Y^{(i) } = h_2( \cZ^{(i)} )  $ is the response of of the mixture of SIMs.
Note that we have
\$
\EE ( \hat M_2) = \EE[ h_2 (\cZ) \cdot    S_3(X) ]  = \sum_{j=1}^k \gamma _j^* \cdot \theta_j ^{* \otimes 3},
\$
where the second equality follows from Lemma \ref{lemma:moments}.   By triangle inequality, we have
\#\label{eq:use_triangle}
\bigl \| \hat M_2 - \EE (\hat M_2)  \bigr \|_{\oper}  \leq \bigl \| \hat T_1 - \EE (\hat T_1)  \bigr \|_{\oper} + \bigl \| \hat T_2- \EE (\hat T_2)  \bigr \|_{\oper}.
\#
In the sequel, we upper bound the two terms on the right-hand of \eqref{eq:use_triangle} separately.
 %\subsubsection{Proof of Equation~\eqref{eq:topt1}}

 %\subsubsection{Proof of Equation~\eqref{eq:topt2}}
 First, since $\hat T_1$ and $\hat T_2$ defined in \eqref{eq:def_T1} and \eqref{eq:def_T2} are symmetric tensors, the definition of tensor operator norm  in \eqref{eq:def_tensor_opernorm} yields that
\#\label{eq:T1_oper_norm_def}
\bigl \| \hat T_1 - \EE ( \hat T_1) \bigr \| _{\oper} =\sup_{u  \in \cS^{d-1}} \Bigl \{ \Bigl | \hat T_1 (u, u, u) - \EE \bigl [  \hat T_1(u,u,u) \bigr ]  \Bigr | \Bigr \},
\#
where $\cS^{d-1} = \{ u \in \RR^d \colon \| u \|_2 = 1 \}$ is the unit sphere in $\RR^d$. Similar to showing the concentration of random matrices, our derivation consists of two steps. In the first step, we  firstly apply the $\epsilon$-net argument  for tensor operator norm.  Then we bound  the concentration of $| \hat T_1(u, u, u) - \EE [ \hat T_1(u,u,u)] |$ for any fixed $u \in \cS^{d-1}$ and apply an union bound over the $\epsilon$-net.

 To begin with, let $N_{\cS} (\epsilon )$ be the $\epsilon$-net of the unit sphere $\cS^{d-1}$ for any $\epsilon \in (0,1)$. We  now
 %
%
%
%{\noindent \bf Step 1.}   We first establish an $\epsilon$-net argument for tensor operator norm. For any set $\cE \subseteq \RR^d$, we say $\cN$  is an $\epsilon$-net for $\cE$, if for any $u \in \cE$, there exists $v \in \cN$ such that $\| u - v \|_2 \leq  \epsilon$.
%The $\epsilon$-net argument is a standard technique for bounding the operator norm of matrices.  In the following lemma, we derive a counterpart for $\ell$-th order  tensors. For an $\ell$-th order tensor $A\in \RR^{d\otimes \ell} $, the operator norm of $A$ is given by
%\#\label{eq:def_tensor_opernorm}
%\| A \|_{\oper} = \sup\bigl \{  \bigl | A(u^{(1)} , \ldots, u^{(\ell)} ) \bigr | \colon  u^{(1)}, u^{(2)}, \ldots, u^{(\ell)} \in \cS^{d-1} \bigr \} .
%\#
 appeal to Lemma~\ref{lem:net}, which shows that  taking  the supremum in \eqref{eq:T1_oper_norm_def} over  $N_{\cS} (1/6)$ instead of $\cS^{d-1}$ only incurs a small error. Specifically, we apply Lemma~\ref{lem:net} with $\ell = 3$, and $\epsilon = 1/6$ to $\hat T_1$ to obtain
\#\label{eq:use_epsilon_argument}
\bigl \| \hat T_1 - \EE ( \hat T_1) \bigr \| _{\oper}  \leq 2 \sup_{u  \in \cN_{\cS}(1/6) } \Bigl \{ \Bigl | \hat T_1 (u, u, u) - \EE \bigl [  \hat T_1(u,u,u) \bigr ]  \Bigr | \Bigr \}.
\#

In the next step, we derive a concentration inequality for  $\hat T_1(u,u,u)$ with fixed  $u \in \cS^{d-1}$, and apply a union bound of $\cN_{\cS}(1/6)$ to conclude the proof.

  By the definition of $\hat T_1$ in \eqref{eq:def_T1}, we have
 we have
\$
\hat T_1(u,u,u) = \frac{1}{n} \sum_{i=1}^n Y^{(i)} \cdot ( X^{(i) \top } u)^3.
\$
By Assumption \ref{assume:moments}, $\{ Y^{(i)} \}_{i\in [n]}$ are i.i.d.   sub-exponential random variables with $\psi_1$-norm bounded by $\Psi$. Moreover, since $\{X^{(i)} \}_{i\in [n]} $ are i.i.d. $ N(0, I_d)$ random vectors, $X^{(i) \top } u$ are independent standard Gaussian random variables for each $u \in \cS^{d-1}$. Thus $\| X^{(i)\top } u \|_{\psi_2} \leq \Upsilon_0$ where $\Upsilon_0 $ is a constant.
To bound $| \hat T_1(u,u,u) - \EE [  \hat T_1 (u,u,u) ] |$, we apply \eqref{eq:third_order_concentration} in Lemma \ref{lemma:sum_sub_exponential} to obtain that
\#\label{eq:apply_third_order}
&\PP \Bigl \{  \Bigl |  \hat T_1(u,u,u) - \EE  \bigl [ \hat T_1 (u, u, u) \bigr ] \Bigr | \geq t  / n\Bigr \}  \leq 4  \exp \Bigl (  - K_1 \cdot \min \big\{    [ t/ (\sqrt{n} \Upsilon_0^3 \cdot \Psi   )  ]^{2},    [ t / ( \Upsilon_0^3 \cdot \Psi )  ] ^{2/5} \bigr\}  \Bigr ),
\#
where $K_1$ is a constant. Moreover, this inequality holds for any $t \geq C_1 \cdot \Upsilon_0^3 \cdot \Psi$, where $C_1$ is a constant. Since both $\Psi$ and $\Upsilon_0$ are constants, we can rewrite \eqref{eq:apply_third_order} as
\#\label{eq:apply2_third_order}
\PP \Bigl \{  \Bigl |  \hat T_1(u,u,u) - \EE  \bigl [ \hat T_1 (u, u, u) \bigr ] \Bigr | \geq t  / n\Bigr \}\leq 4  \exp  \bigl [  - \tilde C \cdot \min \bigl (     t^2 / n,     t  ^{2/5}  \bigr )   \bigr ]  ,
\#
where $\tilde C$ is a constant depending on $\Upsilon_0$ and $\Psi$.  Based on \eqref{eq:apply2_third_order}, we take a union bound over $\cN_{\cS}( 1/6)$.
As shown in    Lemma 5.2 in \cite{vershynin2010introduction}, the capacity of  $\cN_{\cS} (\epsilon) $ is bounded by $(1 + 2/ \epsilon)^{d}$ for any $\epsilon \geq 0$.  Thus we have  $| \cN_{\cS}(1/6) | \leq 13^d$, which implies that
\#\label{eq:union_1}
&\PP \biggl ( \sup_{u \in \cN_{\cS}(1/6)}  \Bigl \{   \Bigl |  \hat T_1(u,u,u) - \EE  \bigl [ \hat T_1 (u, u, u) \bigr ] \Bigr |  \Bigr \}\geq t  / n \biggr )  \leq 4  \exp  \bigl [  - \tilde C \cdot \min \bigl (     t^2 / n,     t  ^{2/5}  \bigr ) + \log 13 \cdot d   \bigr ]  ,
\#
Now we set $  \tilde C \cdot \min  (     t^2 / n,     t  ^{2/5}   ) = 6 d$. Note that $\tilde C$ is a constant. Solving the equation for $t$ yields~that
\#\label{eq:get_t}
t = K_{ 1} / 2 \cdot \max \bigl ( \sqrt{ nd}, d^{5/2} \bigr )
\#
for some constant $K_{ 1}$ depending on $\Psi$ and $\Upsilon_0$.
Finally, combining \eqref{eq:use_epsilon_argument}, \eqref{eq:union_1}, \eqref{eq:get_t}, we conclude that
\#\label{eq:final_t1_bound}
\bigl \| \hat T_1 - \EE ( \hat T_1) \bigr \|_{\oper} \leq K_{ 1} \cdot \max \bigl ( \sqrt{d/n}, d^{5/2} / n \bigr )
\#
holds with probability at least $1 - 4 \exp( -3d)$.

Moreover, for $\hat T_2 $ defined \eqref{eq:def_T2} and any $u \in \cS^{d-1} $, we have
\$
\hat T_2 ( u, u, u) &= \frac{3}{n} \sum_{i=1}^n Y^{(i)} \cdot \sum_{j=1}^d (X^{(i)\top} u)  \cdot (u^\top e_j)^2 \\ &  =  \frac{3}{n} \sum_{i=1}^n Y^{(i)} \cdot (X^{(i)\top}u  )
 \cdot \sum_{j=1}^d  u_j^2    = \frac{3}{n} \sum_{i=1}^n Y^{(i)} \cdot (X^{(i)\top}u  ),
  \$
  where the last equality holds since $\| u \|_2 = 1$.
Note that  $Y^{(i)}$ and $(X^{(i)\top}u  )$ are sub-exponential  and sub-Gaussian random variables, respectively, with $\|X^{(i)\top}u\|_{\psi_2} \leq \Upsilon_0$ and $\| Y \|_{\psi_1} \leq \Psi$.  By  \eqref{eq:third_order_concentration2} in Lemma \ref{lemma:sum_sub_exponential}, we have
\#\label{eq:apply_third_order}
\PP \Bigl \{  \Bigl |  \hat T_2(u,u,u) - \EE  \bigl [ \hat T_2 (u, u, u) \bigr ] \Bigr | \geq t  / n\Bigr \}\leq 4  \exp \Bigl (  - K_2 \cdot \min \big\{    [ t/ (\sqrt{n} \Upsilon_0  \cdot \Psi   )  ]^{2},    [ t / ( \Upsilon_0  \cdot \Psi )  ] ^{2/3} \bigr\}  \Bigr ),
\#
where $K_2 >0 $ is a constant. Then we take a union bound for all $u \in \cN_{\cS} (1/6)$ to obtain that
\#\label{eq:union_2}
\PP \biggl ( \sup_{u \in \cN_{\cS}(1/6)}  \Bigl \{   \Bigl |  \hat T_2(u,u,u) - \EE  \bigl [ \hat T_2 (u, u, u) \bigr ] \Bigr |  \Bigr \}\geq t  / n \biggr )\leq 4  \exp  \bigl [  - \tilde C \cdot \min \bigl (     t^2 / n,     t  ^{2/3}  \bigr ) + \log 13 \cdot d   \bigr ]  ,
\#
where $\tilde C$ is a constant depending on $\Upsilon_0$ and $\Psi$. Similar to \eqref{eq:get_t}, setting $\tilde C \cdot \min  (     t^2 / n,     t  ^{2/3}   ) = 6 d$ implies that
\#\label{eq:get_t2}
t = K_{2} / 2 \cdot \max \bigl ( \sqrt{ nd}, d^{3/2} \bigr )
\#
for some constant $K_{ 2}$. Finally, combining \eqref{eq:union_2} and \eqref{eq:get_t2}, we obtain
\#\label{eq:final_t2_bound}
\bigl \| \hat T_2 - \EE ( \hat T_2) \bigr \|_{\oper} \leq K_{2} \cdot \max \bigl ( \sqrt{d/n}, d^{3/2} / n \bigr )
\#
with probability at least $1 - 4 \exp( -3d)$. Then   combining \eqref{eq:final_t1_bound} and \eqref{eq:final_t2_bound},  we conclude that
\#\label{eq:final_spectral_bound}
\bigl \| \hat M_2 - \EE[ h_2 (\cZ) \cdot    S_3(X) ] \bigr \|_{\oper}  \leq K_{ 1} \cdot \max \bigl ( \sqrt{d/n}, d^{5/2} / n \bigr )
 + K_{ 2} \cdot \max \bigl ( \sqrt{d/n}, d^{3/2} / n \bigr ).
\#
holds with   with probability at least $1 -8 \exp(-3d)$.
  When $d $ is sufficiently large such that $\exp(d) \geq 8$, we conclude that \eqref{eq:final_spectral_bound} holds with probability at least $1 - \exp(-2d)$.





\vspace{10pt}
{\noindent \bf Upper bound for  $\| \hat M_1 - \EE [ h_1(\mathcal{Z}) \cdot S_3(X)]\|_{\oper}$.}
 To conclude the proof, it remains to bound  $\| \hat M_1 - \EE [ h_1(\mathcal{Z}) \cdot S_3(X)]\|_{\oper}$.  For notational simplicity,   we denote  $ h_1(\cZ^{(i)} ) = k^{-1} \sum_{j\in [k]} Z_j^{(i)} $ by $W^{(i) } $ for any $i \in [n]$.  Then by \eqref{eq:moment_tensor1},  we can write  $\hat M_1 = \sum_{i =1}^n W^{(i) } \cdot S_3(X^{(i)}) = \hat T_3  +\hat T_4$, where we define $\hat T_3$ and $\hat T_4$ respectively~by
\#
& \hat T_3 = \frac{1}{n} \sum_{i=1}^n W^{(i)}  \cdot X^{(i)} \otimes X^{(i)} \otimes X^{(i)}, \label{eq:def_T4} \\
& \hat T_4 = \frac{1}{n} \sum_{i=1}^n \sum_{j=1}^d W^{(i)}  \cdot \bigl  ( X^{(i)} \otimes e_j \otimes e_j +e_j \otimes X^{(i)}\otimes e_j + e_j \otimes e_j \otimes X^{(i)} \bigr ) \label{eq:def_T4}.
\#
We note that here the $\hat T_3$ and $\hat T_4$ is defined in the same fashion as $\hat T_1$ and $\hat T_2$ defined in   \eqref{eq:def_T1} and \eqref{eq:def_T2} with $\{Y^{(i)} \}_{i\in [n]}$ replaced by $\{W^{(i)} \}_{i\in [n]}$.
Then triangle inequality implies that
\#\label{eq:use_triangle2}
\bigl \| \hat M_1 -  \EE [ h_1(\mathcal{Z}) \cdot S_3(X)]  \bigr \|_{\oper}  \leq \bigl \| \hat T_3 - \EE (\hat T_3)  \bigr \|_{\oper} + \bigl \| \hat T_4- \EE (\hat T_4)  \bigr \|_{\oper}.
\#
Moreover, by Assumption \ref{assume:moments}, we have $\| Z_j \| _{\psi_1} \leq \Psi$ for each $j\in [k]$.  We   appeal to  Lemma \ref{lemma:psi_1_norm} to obtain  that $\| h_1(\cZ) \|_{\psi_1} \leq \Psi$, which implies that
$\| W^{(i) } \| _{\psi_1} \leq \Psi$ for any $i \in [n]$.
Thus, following the same derivation for \eqref{eq:final_spectral_bound} with $Y^{(i)}$ replaced by $W^{(i)}$ for all $i\in [n]$, we obtain that
\#\label{eq:final_spectral_bound2}
\bigl \| \hat M_1 - \EE[ h_1 (\cZ) \cdot    S_3(X) ] \bigr \|_{\oper}  \leq K_{ 1} \cdot \max \bigl ( \sqrt{d/n}, d^{5/2} / n \bigr )
 + K_{ 2} \cdot \max \bigl ( \sqrt{d/n}, d^{3/2} / n \bigr ).
\#
with probability at least $1- \exp(-2d)$. Here the constants $K_1$ and $K_2$ are given in \eqref{eq:get_t} and \eqref{eq:get_t2}, respectively.
Finally, combining \eqref{eq:final_spectral_bound} and \eqref{eq:final_spectral_bound2}, we conclude the proof of Theorem \ref{thm:tensor_concentration}.





\input{sparse_tensor}



